Designing Fairness in Autonomous Peer-to-peer Energy Trading

Several autonomous energy management and peer-to-peer trading mechanisms for future energy markets have been recently proposed based on optimization and game theory. In this paper, we study the impact of trading prices on the outcome of these market designs for energy-hub networks. We prove that, for a generic choice of trading prices, autonomous peer-to-peer trading is always network-wide beneficial but not necessarily individually beneficial for each hub. Therefore, we leverage hierarchical game theory to formalize the problem of designing locally-beneficial and network-wide fair peer-to-peer trading prices. Then, we propose a scalable and privacy-preserving price-mediation algorithm that provably converges to a profile of such prices. Numerical simulations on a 3-hub network show that the proposed algorithm can indeed incentivize active participation of energy hubs in autonomous peer-to-peer trading schemes.

==> 23 - VE BEL - ECC/macros.tex <==
%% macros

\usepackage{color}
\usepackage{enumerate,graphicx,epstopdf}
\usepackage{amsmath,amssymb,bm}
\usepackage{cite}
\usepackage{mathtools}
\usepackage{array}
\usepackage{algpseudocode,algorithm,algorithmicx}
\usepackage{color}
\usepackage{booktabs}
\usepackage[hyphens]{url}
\usepackage{lipsum}
 \usepackage[dvipsnames]{xcolor}
\usepackage[deletedmarkup=sout,authormarkup=superscript]{changes}
\usepackage[normalem]{ulem}
\usepackage{flushend}
\newcommand\at[2]{\left.#1\right|_{#2}}

% Bibliography Properties
\bibliographystyle{ieeetr}

\newtheorem{ass}{Assumption}
\newtheorem{rmk}{Remark}
\newtheorem{dfn}{Definition}
\newtheorem{lmm}{Lemma}
\newtheorem{prp}{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{thm}{Theorem}
\newtheorem{ex}{Example}

\newcommand{\ints}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand\intrng[2]{\ints_{[#1,#2]}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\sqr}{$\hfill\square$}
\newcommand{\gph}{\mathrm{gph}~}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\Int}[0]{\mathrm{Int}~}
\renewcommand{\ker}[0]{\mathrm{Ker}~}
\renewcommand{\Im}[0]{\mathrm{Im}~}
\newcommand{\prox}[0]{\mathrm{prox_V^{\gamma}}}
\newcommand{\dist}[0]{\mathrm{dist}}
\newcommand{\dom}[0]{\mathrm{Dom}~}
\newcommand{\col}{\mathrm{col}}

\newcommand{\esssup}[0]{\overline{\sup}}

\def\red{\textcolor{red}}
\def\blue{\textcolor{blue}}
\def\green{\textcolor{green}}

\newcommand\veps[0]{\varepsilon}
\newcommand\eps[0]{\epsilon}
\newcommand\oh[0]{o}
\newcommand\Oh[0]{\mathcal{O}}

\newcommand\Kinf[0]{\mathcal{K}_\infty}
\newcommand\KL[0]{\mathcal{KL}}
\newcommand\K[0]{\mathcal{K}}
\renewcommand\L[0]{\mathcal{L}}
\newcommand\limsupk[0]{\underset{k\to\infty}{\overline{\lim}}}
\newcommand\sig[0]{\mathbb{L}}

\newcommand{\mto}[0]{\rightrightarrows}
% \newcommand{\defeq}[0]{\overset{\Delta}{=}}
\newcommand{\defeq}[0]{\equiv}
%\newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin}}}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\kto}[0]{\xrightarrow{k\rightarrow\infty}}

\newcommand{\nc}{\mathcal{N}}
\newcommand{\proj}{\mathrm{proj}}
\newcommand\id[0]{\mathrm{id}}
\newcommand{\fix}{\mathrm{fix}}
\newcommand{\zer}{\mathrm{zer}}

\definechangesauthor[name={Giuseppe}, color=NavyBlue]{GB}
\definechangesauthor[name={Varsha}, color=RedViolet]{VB}


\newcommand{\gb}[1] {\added[id=GB]{[#1]}}
\newcommand{\dlm}[1] {\added[id=DLM]{[#1]}}
\newcommand{\mhd}[1] {\added[id=MHD]{[#1]}}

==> macros.tex <==
%% macros

%\usepackage{color}
\usepackage{enumerate,graphicx,epstopdf}
\usepackage{amsmath,amssymb,bm}
\usepackage{cite}
\usepackage{mathtools}
\usepackage{array}
\usepackage{algpseudocode,algorithm,algorithmicx}
\usepackage{booktabs}
\usepackage[hyphens]{url}
\usepackage{lipsum}
% \usepackage[dvipsnames]{xcolor}
\usepackage[deletedmarkup=sout,authormarkup=superscript]{changes}
\usepackage[normalem]{ulem}
\usepackage{flushend}
\newcommand\at[2]{\left.#1\right|_{#2}}

% Bibliography Properties
%\bibliographystyle{ieeetr}

%\newtheorem{ass}{Assumption}
%\newtheorem{rmk}{Remark}
%\newtheorem{dfn}{Definition}
%\newtheorem{lmm}{Lemma}
%\newtheorem{prp}{Proposition}
%\newtheorem{cor}{Corollary}
%\newtheorem{thm}{Theorem}
%\newtheorem{ex}{Example}

\newcommand{\ints}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand\intrng[2]{\ints_{[#1,#2]}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\sqr}{$\hfill\square$}
\newcommand{\gph}{\mathrm{gph}~}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\Int}[0]{\mathrm{Int}~}
\renewcommand{\ker}[0]{\mathrm{Ker}~}
\renewcommand{\Im}[0]{\mathrm{Im}~}
\newcommand{\prox}[0]{\mathrm{prox_V^{\gamma}}}
\newcommand{\dist}[0]{\mathrm{dist}}
\newcommand{\dom}[0]{\mathrm{Dom}~}
\newcommand{\col}{\mathrm{col}}

\newcommand{\esssup}[0]{\overline{\sup}}

%\def\red{\textcolor{red}}
%\def\blue{\textcolor{blue}}
%\def\green{\textcolor{green}}

\newcommand\veps[0]{\varepsilon}
\newcommand\eps[0]{\epsilon}
\newcommand\oh[0]{o}
\newcommand\Oh[0]{\mathcal{O}}

\newcommand\Kinf[0]{\mathcal{K}_\infty}
\newcommand\KL[0]{\mathcal{KL}}
\newcommand\K[0]{\mathcal{K}}
\renewcommand\L[0]{\mathcal{L}}
\newcommand\limsupk[0]{\underset{k\to\infty}{\overline{\lim}}}
\newcommand\sig[0]{\mathbb{L}}

\newcommand{\mto}[0]{\rightrightarrows}
% \newcommand{\defeq}[0]{\overset{\Delta}{=}}
\newcommand{\defeq}[0]{\equiv}
%\newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin}}}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\kto}[0]{\xrightarrow{k\rightarrow\infty}}

\newcommand{\nc}{\mathcal{N}}
\newcommand{\proj}{\mathrm{proj}}
\newcommand\id[0]{\mathrm{id}}
\newcommand{\fix}{\mathrm{fix}}
\newcommand{\zer}{\mathrm{zer}}
%
%\definechangesauthor[name={Giuseppe}, color=blue]{GB}
%\definechangesauthor[name={Varsha}, color=red]{VB}
%
%
%\newcommand{\gb}[1] {\added[id=GB]{[#1]}}
%\newcommand{\vb}[1] {\added[id=VB]{[#1]}}


==> old/ecc/macros.tex <==
%% macros

%\usepackage{color}
\usepackage{enumerate,graphicx,epstopdf}
\usepackage{amsmath,amssymb,bm}
\usepackage{cite}
\usepackage{mathtools}
\usepackage{array}
\usepackage{algpseudocode,algorithm,algorithmicx}
\usepackage{booktabs}
\usepackage[hyphens]{url}
\usepackage{lipsum}
% \usepackage[dvipsnames]{xcolor}
\usepackage[deletedmarkup=sout,authormarkup=superscript]{changes}
\usepackage[normalem]{ulem}
\usepackage{flushend}
\newcommand\at[2]{\left.#1\right|_{#2}}

% Bibliography Properties
%\bibliographystyle{ieeetr}

%\newtheorem{ass}{Assumption}
%\newtheorem{rmk}{Remark}
%\newtheorem{dfn}{Definition}
%\newtheorem{lmm}{Lemma}
%\newtheorem{prp}{Proposition}
%\newtheorem{cor}{Corollary}
%\newtheorem{thm}{Theorem}
%\newtheorem{ex}{Example}

\newcommand{\ints}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand\intrng[2]{\ints_{[#1,#2]}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\sqr}{$\hfill\square$}
\newcommand{\gph}{\mathrm{gph}~}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\Int}[0]{\mathrm{Int}~}
\renewcommand{\ker}[0]{\mathrm{Ker}~}
\renewcommand{\Im}[0]{\mathrm{Im}~}
\newcommand{\prox}[0]{\mathrm{prox_V^{\gamma}}}
\newcommand{\dist}[0]{\mathrm{dist}}
\newcommand{\dom}[0]{\mathrm{Dom}~}
\newcommand{\col}{\mathrm{col}}

\newcommand{\esssup}[0]{\overline{\sup}}

%\def\red{\textcolor{red}}
%\def\blue{\textcolor{blue}}
%\def\green{\textcolor{green}}

\newcommand\veps[0]{\varepsilon}
\newcommand\eps[0]{\epsilon}
\newcommand\oh[0]{o}
\newcommand\Oh[0]{\mathcal{O}}

\newcommand\Kinf[0]{\mathcal{K}_\infty}
\newcommand\KL[0]{\mathcal{KL}}
\newcommand\K[0]{\mathcal{K}}
\renewcommand\L[0]{\mathcal{L}}
\newcommand\limsupk[0]{\underset{k\to\infty}{\overline{\lim}}}
\newcommand\sig[0]{\mathbb{L}}

\newcommand{\mto}[0]{\rightrightarrows}
% \newcommand{\defeq}[0]{\overset{\Delta}{=}}
\newcommand{\defeq}[0]{\equiv}
%\newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin}}}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\kto}[0]{\xrightarrow{k\rightarrow\infty}}

\newcommand{\nc}{\mathcal{N}}
\newcommand{\proj}{\mathrm{proj}}
\newcommand\id[0]{\mathrm{id}}
\newcommand{\fix}{\mathrm{fix}}
\newcommand{\zer}{\mathrm{zer}}
%
%\definechangesauthor[name={Giuseppe}, color=blue]{GB}
%\definechangesauthor[name={Varsha}, color=red]{VB}
%
%
%\newcommand{\gb}[1] {\added[id=GB]{[#1]}}
%\newcommand{\vb}[1] {\added[id=VB]{[#1]}}


==> table.tex <==

\begin{table}[H]
    \centering
    \begin{tabular}{ |c|c|c|c| } 
    \hline
    \textbf{Hub component} & \textbf{Parameters} & \textbf{Values}\\
    \hline 
    \multirow{2}{2em}{PV} & $\eta_{PV}$ & $0.15$ \\
    & $A$ & $2538 m^2$ \\
    \hline 
    \multirow{2}{2em}{HP} & $\eta_{HP}$ & $4.5$ \\
    & $Q_{HP}^{max}$ & $350kW$ \\
    \hline 
    \multirow{11}{2em}{CHP} & $\eta_{CHP}$ & $0.36$ \\
    & $P_1$ & $0kW$ \\
    & $P_2$ & $317kW$ \\
    & $P_3$ & $754kW$ \\
    & $P_4$ & $437kW$ \\
    & $P_5$ & $111kW$ \\
    & $Q_1$ & $0kW$ \\
    & $Q_2$ & $513kW$ \\
    & $Q_3$ & $1220kW$ \\
    & $Q_4$ & $707kW$ \\
    & $Q_5$ & $0kW$ \\
    \hline 
    \multirow{5}{2em}{mCHP} & $\eta_{mCHP}$ & $0.34$ \\
    & $E_{mCHP}^{min}$ & $0 kW$ \\
    & $E_{mCHP}^{min}$ & $240 kW$ \\
    & $\alpha_{mCHP}^P$ & $0.38$ \\
    & $\alpha_{mCHP}^Q$ & $0.62$ \\
    \hline
    \multirow{2}{2em}{GB} & $\eta_{GB}$ & $0.87$ \\
    & $Q_{GB}^{max}$ & $350kW$ \\
    \hline 
    \multirow{6}{2em}{B} & $\eta_{B}$ & $0.999$ \\
    & $\eta_{B}$ & $0.99$ \\
    & $E_{B}^{ini}$ & $252 kW$ \\
    & $E_{B}^{min}$ & $42 kW$ \\
    & $E_{B}^{max}$ & $757 kW$ \\
    & $\gamma_{B}$ & $0.25$ \\
    \hline
    \multirow{6}{2em}{HT} & $\eta_{B}$ & $0.992$ \\
    & $\eta_{HT}$ & $0.99$ \\
    & $E_{HT}^{ini}$ & $4301 kW$ \\
    & $E_{HT}^{min}$ & $ 2867kW$ \\
    & $E_{HT}^{max}$ & $12904 kW$ \\
    & $\gamma_{HT}$ & $0.25$ \\
    \hline
    \end{tabular}
    \caption{Hub 1: Component Parameters}
    \label{tab:hub 1}
\end{table}


\begin{table}[H]
    \centering
    \begin{tabular}{ |c|c|c|c| } 
    \hline
    \textbf{Hub component} & \textbf{Parameters} & \textbf{Values}\\
    \hline 
    \multirow{2}{2em}{PV} & $\eta_{PV}$ & $0.15$ \\
    & $A$ & $9540 m^2$ \\
    \hline 
    \multirow{2}{2em}{HP} & $\eta_{HP}$ & $4.5$ \\
    & $Q_{HP}^{max}$ & $400kW$ \\
    \hline 
    \multirow{2}{2em}{GB} & $\eta_{GB}$ & $0.87$ \\
    & $Q_{GB}^{max}$ & $50kW$ \\
    \hline 
    \multirow{6}{2em}{HT} & $\eta_{B}$ & $0.992$ \\
    & $\eta_{HT}$ & $0.99$ \\
    & $E_{HT}^{ini}$ & $0.54 kW$ \\
    & $E_{HT}^{min}$ & $ 0.36kW$ \\
    & $E_{HT}^{max}$ & $1.62 kW$ \\
    & $\gamma_{HT}$ & $0.25$ \\
    \hline
    \end{tabular}
    \caption{Hub 2: Component Parameters}
    \label{tab:hub 2}
\end{table}


\begin{table}[H]
    \centering
    \begin{tabular}{ |c|c|c|c| } 
    \hline
    \textbf{Hub component} & \textbf{Parameters} & \textbf{Values}\\
    \hline 
    \multirow{2}{2em}{PV} & $\eta_{PV}$ & $0.15$ \\
    & $A$ & $ 1160m^2$ \\
    \hline 
    \multirow{2}{2em}{HP} & $\eta_{HP}$ & $4.5$ \\
    & $Q_{HP}^{max}$ & $50kW$ \\
    \hline 
    \end{tabular}
    \caption{Hub 3: Component Parameters}
    \label{tab:hub 3}
\end{table}
